BEV-TSR: Text-Scene Retrieval in BEV Space for Autonomous Driving

The rapid development of the autonomous driving industry has led to a significant accumulation of autonomous driving data. Consequently, there comes a growing demand for retrieving data to provide specialized optimization. However, directly applying previous image retrieval methods faces several challenges, such as the lack of global feature representation and inadequate text retrieval ability for complex driving scenes. To address these issues, firstly, we propose the BEV-TSR framework which leverages descriptive text as an input to retrieve corresponding scenes in the Bird's Eye View (BEV) space. Then to facilitate complex scene retrieval with extensive text descriptions, we employ a large language model (LLM) to extract the semantic features of the text inputs and incorporate knowledge graph embeddings to enhance the semantic richness of the language embedding. To achieve feature alignment between the BEV feature and language embedding, we propose Shared Cross-modal Embedding with a set of shared learnable embeddings to bridge the gap between these two modalities, and employ a caption generation task to further enhance the alignment. Furthermore, there lack of well-formed retrieval datasets for effective evaluation. To this end, we establish a multi-level retrieval dataset, nuScenes-Retrieval, based on the widely adopted nuScenes dataset. Experimental results on the multi-level nuScenes-Retrieval show that BEV-TSR achieves state-of-the-art performance, e.g., 85.78% and 87.66% top-1 accuracy on scene-to-text and text-to-scene retrieval respectively. Codes and datasets will be available.

==> latex/tab/RDF.tex <==
\begin{wraptable}{r}{8.5cm}
  \centering 
   \addtolength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{l l l}
  \toprule
\textbf{Subject} & \textbf{Predicate}   & \textbf{Object}  \\ \midrule
inst:scene       & rdf:type             & Object:Scene     \\
inst:scene       & rdf:includeType      & Object:Vehicle   \\
inst:scene       & rdf:include          & inst:vehicle     \\
inst:vehicle     & rdf:participate\_in  & inst:driving     \\
inst:driving     & rdf:type             & Movement:Driving \\
inst:vehicle     & rdf:participate\_in  & inst:driving     \\
inst:driving     & rdf:has\_participant & inst:vehicle     \\ \bottomrule
\end{tabularx}
\caption{\textbf{Example Resource Description Frameworks (RDF) in autonomous driving knowledge graph \Tao{inst? rdf?}} }
\label{tab: rdf}

\end{wraptable}

==> latex/tab/ablation_caption.tex <==
\begin{table*}[ht]
  \centering 
   \addtolength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{l|cc|cccccc}
\toprule 
 Method    & CG & Distmult                          & B2T\_R1        & B2T\_R5        & B2T\_R10       & T2B\_R1         & T2B\_R5         & T2B\_R10        \\ \midrule
\multirow{4}*{Llama baseline}     & -- & --          & 0.8552          & \textbf{0.9944} & 0.9988          & 0.8731          & 0.9962          & 0.9991          \\
     & $\checkmark$ & --        & \textbf{0.8573} & 0.9930          & \textbf{0.9988} & \textbf{0.8751} & \textbf{0.9974} & \textbf{0.9991} \\ \cline{2-9}
   & -- & $\checkmark$    & \textbf{0.8599} & 0.9947          & 0.9994          & 0.8757          & 0.9968          & 0.9994          \\
  & $\checkmark$ & $\checkmark$ & 0.8578          & \textbf{0.9954} & \textbf{0.9994} & \textbf{0.8766} & \textbf{0.9971} & \textbf{0.9997} \\ 
\bottomrule 
\end{tabularx}
\caption{Ablation study results of adding caption generation as an auxiliary task. CG refers to the model trained with cation generation head. Llama baseline includes : Llama2* + LoRA + SCP.}
\label{tab: ablation_caption}
\vspace{-1em}
\end{table*}


==> latex/tab/ablation_caption_2.tex <==
\begin{table*}[ht]
  \centering 
   \addtolength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{l|cc|cccccc}
\toprule 
 Method    & CG & Distmult                          & B2T\_R1        & B2T\_R5        & B2T\_R10       & T2B\_R1         & T2B\_R5         & T2B\_R10        \\ \midrule
\multirow{4}*{Llama baseline}     & -- & --          & 0.6552 & 0.9877          & 0.9988          & 0.6631          & 0.9871          & 0.9991          \\
   & -- & $\checkmark$    & 0.6602          & 0.9848          & 0.9985          & 0.6719          & 0.9865          & 0.9994          \\
  & $\checkmark$ & $\checkmark$ & 0.6608          & \textbf{0.9912} & \textbf{0.9997} & \textbf{0.6790} & \textbf{0.9862} & \textbf{0.9991} \\ 
\bottomrule 
\end{tabularx}
\caption{Ablation study results of adding caption generation as an auxiliary task with augmented NuScenes-QA data. CG refers to the model trained with cation generation head. Llama baseline includes : Llama2* + LoRA + SCP.}
\label{table: ablation_caption_2}
\vspace{-1em}
\end{table*}

==> latex/tab/ablation_kg.tex <==
\begin{table*}[ht]
  \centering 
   \addtolength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{c|cccccc}
\toprule 
   KGE                     & B2T\_R1        & B2T\_R5        & B2T\_R10       & T2B\_R1         & T2B\_R5         & T2B\_R10        \\ \midrule 
   --      & 0.7875          & 0.9757          & 0.9909          & 0.8194          & 0.9812          & 0.9906          \\
   TransE & 0.8009          & 0.9804          & 0.9936          & 0.8455          & 0.9892          & 0.9965          \\
  Distmult & \textbf{0.8059} & \textbf{0.9783} & 0.9947          & \textbf{0.8584} & \textbf{0.9909} & 0.9959          \\
     ConvE    & 0.8050          & 0.9780          & \textbf{0.9956} & 0.8473          & 0.9889          & \textbf{0.9968} \\ 
\bottomrule 
\end{tabularx}
\caption{Ablation study results when using different knowledge graph. * denotes that the model parameters are frozen. KGE refers to knowledge graph embedding \Tao{please ablate on the whole method }}
\label{tab: ablation_kg}
\end{table*}
% baseline + KG

==> latex/tab/ablation_kg_2.tex <==
\begin{table*}[ht]
  \centering 
   \addtolength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{l|c|cccccc}
\toprule 
Method  & KGE                     & B2T\_R1        & B2T\_R5        & B2T\_R10       & T2B\_R1         & T2B\_R5         & T2B\_R10        \\ \midrule
\multirow{4}*{Llama2* + LoRA} & --       & 0.5339          & 0.9355          & 0.9742          & 0.5476          & 0.9472          & 0.9848          \\
   &TransE & 0.5497          & 0.9420          & 0.9760          & 0.5676          & 0.9396          & 0.9716          \\
  & Distmult & 0.5456 & 0.9387 & 0.9733          & 0.5644 & 0.9305 & 0.9678          \\
  & ConvE    & 0.5582          & 0.9343          & 0.9730 & 0.5620          & 0.9343          & 0.9713 \\ 
\bottomrule 
\end{tabularx}
\caption{Ablation study results when using different knowledge graph with augmented NuScenes-QA data. * denotes that the model parameters are frozen. KGE refers to knowledge graph embedding}
\label{table: ablation_kg_2}
\end{table*}

==> latex/tab/ablation_nusqa.tex <==
\begin{table*}[ht]
  \centering 
   \addtolength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{l|cccc|cccccc}
\toprule 
 Method      & LoRA &    SCP & KG & CG                                    & B2T\_R1        & B2T\_R5        & B2T\_R10       & T2B\_R1         & T2B\_R5         & T2B\_R10        \\ \midrule
BERT*     & -- & --  &  -- & --                          & 0.3835          & 0.8305          & 0.9109          & 0.3415          & 0.7842          & 0.8687          \\
\midrule
\multirow{4}*{Llama2*}    &$\checkmark$       & -- & --  &  --                                 & 0.5339          & 0.9355          & 0.9742          & 0.5476          & 0.9472          & 0.9848          \\
~   &$\checkmark$       & $\checkmark$ & --  &  --      & 0.6552 & 0.9877          & 0.9988          & 0.6631          & 0.9871          & 0.9991          \\
~  &$\checkmark$       & $\checkmark$ & $\checkmark$  &  --       & \textbf{0.6637}          & 0.9865          & 0.9991          & 0.6637          & 0.9877          & 0.9985          \\
~  &$\checkmark$       & $\checkmark$ & $\checkmark$  &  $\checkmark$   & 0.6608          & \textbf{0.9912} & \textbf{0.9997} & \textbf{0.6790} & \textbf{0.9862} & \textbf{0.9991} \\ 
\bottomrule 
\end{tabularx}
\caption{Comparison of all results on NuScenes-QA augmented data. * denotes that the model parameters are frozen, SCP refers to shared cross-modal prompt, KG refers to Distmult knowledge graph embeddings, and CG refers to caption generation head. }
\label{table: ablation_nusqa}
\end{table*}


==> latex/tab/ablation_scp.tex <==
\begin{table*}[ht]
  \centering 
   \addtolength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{l|cccc|cccccc}
\toprule 
  Method                                          & LoRA & MLP & SCP & Distmult & B2T\_R1        & B2T\_R5        & B2T\_R10       & T2B\_R1         & T2B\_R5         & T2B\_R10        \\ \midrule
\multirow{6}*{Llama2*} & -- & $\checkmark$  &  -- & --                              & 0.7244          & 0.9472          & 0.9713          & 0.7030          & 0.9507          & 0.9730          \\
  & -- & --  &  $\checkmark$ & --                  & \textbf{0.8291} & \textbf{0.9938} & \textbf{0.9997} & \textbf{0.8247} & \textbf{0.9959} & \textbf{1.0000} \\\cline{2-11}
  & $\checkmark$ & $\checkmark$  &  -- & --                       & 0.7875          & 0.9757          & 0.9909          & 0.8194          & 0.9812          & 0.9906          \\
  & $\checkmark$ & --  &  $\checkmark$ & --            & \textbf{0.8552} & \textbf{0.9944} & \textbf{0.9988} & \textbf{0.8751} & \textbf{0.9962} & \textbf{0.9991} \\ \cline{2-11}
  & $\checkmark$ & --  &  -- & $\checkmark$                  & 0.8059          & 0.9783          & 0.9947          & 0.8584          & 0.9909          & 0.9959          \\
  & $\checkmark$ & --  &  $\checkmark$ & $\checkmark$ & \textbf{0.8599} & \textbf{0.9947} & \textbf{0.9994} & \textbf{0.8757} & \textbf{0.9968} & \textbf{0.9994} \\ 
\bottomrule 
\end{tabularx}
\caption{Ablation study results of adding SCP when using multiple different baselines.* denotes that the model parameters are frozen, SCP refers to shared multi-modal prompt}
\label{tab: ablation_scp}
\end{table*}


==> latex/tab/ablation_text_encoder.tex <==
\begin{table*}[ht]
  \centering 
   \addtolength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{l|cc|cccccc}
\toprule 
 Method                    &MLP & LoRA  & B2T\_R1        & B2T\_R5        & B2T\_R10       & T2B\_R1         & T2B\_R5         & T2B\_R10        \\ \midrule
BERT*      & -- & --  & 0.6409          & 0.9129          & 0.9557          & 0.5594          & 0.8915          & 0.9384          \\ \midrule
\multirow{2}*{Llama2*}        &$\checkmark$ & --  & 0.7244          & 0.9472          & 0.9713          & 0.7030          & 0.9507          & 0.9730          \\
  &$\checkmark$ & $\checkmark$  & \textbf{0.7875} & \textbf{0.9757} & \textbf{0.9909} & \textbf{0.8194} & \textbf{0.9812} & \textbf{0.9906} \\ 
\bottomrule 
\end{tabularx}
\caption{Ablation study results when using different text encoder. * denotes that the model parameters are frozen. \Tao{please ablate on the whole method }}
\label{tab: ablation_text_encoder}
\end{table*}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


